Power deposition studies for standard and crystal-assisted heavy ion collimation inthe CERN Large Hadron Collider

The LHC heavy-ion program with $^{208}$Pb$^{82+}$ beams will benefit from a significant increase of the beam intensity when entering its High-Luminosity era in Run~3 (2023). The stored energy is expected to surpass 20~MJ per beam. The LHC is equipped with a betatron collimation system, which intercepts the transverse beam halo and protects sensitive equipment such as superconducting magnets against beam losses. However, nuclear fragmentation and electromagnetic dissociation of $^{208}$Pb$^{82+}$ ions in collimators generates a flux of secondary fragments, which are lost in downstream dispersion suppressor and arc cells. These secondary ions may pose a performance limitation in upcoming runs since they can induce magnet quenches. In order to mitigate this risk, an alternative collimation technique, relying on bent crystals as primary collimators, will be used in forthcoming heavy-ion runs. In this paper, we study the power deposition in superconducting magnets by means of tracking and \textsc{FLUKA} shower simulations, comparing the standard collimation system against the crystal-based one. In order to quantify the predictive ability of the simulation model, we present absolute benchmarks against beam loss monitor measurements from the 2018 $^{208}$Pb$^{82+}$ run at 6.37~$Z$TeV. The benchmarks cover several hundred meters of beamline, from the primary collimators to the first arc cells. Based on these studies, we provide a detailed analysis of ion fragmentation and leakage to the cold magnets and quantify the expected quench margin in future $^{208}$Pb$^{82+}$ runs.

==> Classification.tex <==
Classification (PhySH)

Research Areas -> Beam techniques -> Collimation
Research Areas -> Particle phenomena -> Particle interaction

Physical Systems -> Accs and storage rings -> High-energy accs & colliders -> Colliders -> Hadron colliders
Physical systems -> Accs subsystems -> Machine Protection

Techniques -> Computational Techniques -> Monte Carlo methods

==> Letter_editor.tex <==
Dear Editor,

The LHC heavy-ion program with $^{208}$Pb$^{82+}$ beams will benefit from a significant increase of the beam intensity when entering its High-Luminosity era in Run~3 (2023). Nuclear fragmentation and electromagnetic dissociation of $^{208}$Pb$^{82+}$ ions in collimators jaws generates a flux of secondary fragments, which are lost in downstream dispersion suppressor and arc cells. These secondary ions can induce magnet quenches, posing a performance limitation in upcoming highly energetic runs.

In this paper, we study the power deposition in superconducting magnets by means of particle tracking and \textsc{FLUKA} shower simulations, comparing the standard collimation system against a newly crystal-based one. The new collimation technique rely on bent crystals as primary collimators, to improve the overall performance of the LHC heavy-ion program.
We present absolute benchmarks of the simulations against beam loss monitor measurements from the 2018 $^{208}$Pb$^{82+}$ run at 6.37~$Z$TeV, which cover several hundred meters of beamline. A remarkable agreement between the simulations and measurements is found, which enables more accurate predictions for future runs with higher-intensity beams.
We also provide a detailed analysis of the particle leakage to the cold magnets and show that the crystal-based collimation system can provide a satisfactory reduction of the power density in superconducting magnets.

Overall, the results of this study provides important insights into the performance of the betatron halo collimation system for heavy-ion beams at the LHC. They are essential for the upcoming High-Luminosity heavy-ion runs, which will have a stored energy surpassing 20~MJ per beam. 

Kind regards,

Jean-Baptiste Potoine

European Organization for Nuclear Research (CERN),
Espl. des Particules 1,
1211 Geneva,
Switzerland
